Demystifying Mobile Web Browsing under Multiple Protocols

With the popularity of mobile devices, such as smartphones, tablets, users prefer visiting Web pages on mobile devices. Meanwhile, HTTP(S) plays as the major protocol to deliver Web contents, and has served the Web well for more than 15 years. However, as the Web pages grow increasingly complex to provide more content and functionality, the shortcomings and inflexibility of HTTP become more and more urgent to solve, e.g., the sluggish page load, insecure content, redundant transfer, etc. SPDY and HTTP/2 are promoted to solve the shortcomings and inflexibilities of HTTP/1.x. We are interested in how Web pages perform on smartphones with different protocols, including HTTP, HTTPS, SPDY, and HTTP/2. In this paper, we divide our experiments into two parts. First, in order to simplify our analysis, we develop our own HTTP client ignoring complicated process in real browsers to fetch synthetic Web pages with pre-specified object sizes and object numbers with different protocols, respectively. Meanwhile, we emulate different network conditions between client and server using Traffic Control. In order to test with real browsers, we clone Alexa top 200 websites, which have the corresponding mobile version, into our local host. Meanwhile, we control mobile Chrome browser to load those Web pages with different protocols and emulate different network conditions using Traffic Control. We identify how Web page characteristics and network conditions affect Web performance on smartphones for each protocol. We also conduct experiments on a low-end device to observe if a less powerful processor could affect Web page performance for each protocol.

==> section/biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/Xuanzhe}}]{Xuanzhe~Liu}
is an associate professor in the School of Electronics Engineering
and Computer Science, Peking University, Beijing, China. His research interests
are in the area of services computing, mobile computing, web-based systems, and big data analytic.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/liuyi}}]{Yi Liu} is a Ph.D. student from Peking University majoring in computer science and technology. His research interests include mobile network and systems.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/mayun}}]{Yun~Ma}
is a Ph.D student in the School of Electronics Engineering
and Computer Science of Peking University, Beijing, China.  His research interests include services computing and web engineering.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1.2in,height=1.25in,clip,keepaspectratio]{figure/yunxin}}]{Yunxin~Liu} is a lead researcher in Microsoft Research Asia. He received my Ph.D. in computer science from Shanghai Jiao Tong University in 2011 (through the SJTU-MSRA joint PhD program). His current research interests include mobile systems and networking.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/Huanggang}}]{Gang~Huang} is now
a full professor in Institute of Software, Peking University.
His research interests are in the area of middleware of cloud computing and mobile computing. He is a member of IEEE.
\end{IEEEbiography}


%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/meihong}}]{Hong~Mei}
%is a full professor of School of Electronics Engineering and
%Computer Science, Peking University, Beijing, China. His current research interests are in the area of software engineering and operating systems.
%Hong Mei is a member of the Expert Committee for Information Technology of State 863 High-Tech Program, a chief scientist of State 973 Fundamental Research Program. He is the Member of Chinese Academy of Sciences, and the Fellow of China Computer Federation (CCF). He is a fellow of the IEEE.
%\end{IEEEbiography}

